MOFormer: Self-Supervised Transformer model for Metal-Organic Framework Property Prediction

Metal-Organic Frameworks (MOFs) are materials with a high degree of porosity that can be used for applications in energy storage, water desalination, gas storage, and gas separation. However, the chemical space of MOFs is close to an infinite size due to the large variety of possible combinations of building blocks and topology. Discovering the optimal MOFs for specific applications requires an efficient and accurate search over an enormous number of potential candidates. Previous high-throughput screening methods using computational simulations like DFT can be time-consuming. Such methods also require optimizing 3D atomic structure of MOFs, which adds one extra step when evaluating hypothetical MOFs. In this work, we propose a structure-agnostic deep learning method based on the Transformer model, named as MOFormer, for property predictions of MOFs. The MOFormer takes a text string representation of MOF (MOFid) as input, thus circumventing the need of obtaining the 3D structure of hypothetical MOF and accelerating the screening process. Furthermore, we introduce a self-supervised learning framework that pretrains the MOFormer via maximizing the cross-correlation between its structure-agnostic representations and structure-based representations of crystal graph convolutional neural network (CGCNN) on >400k publicly available MOF data. Using self-supervised learning allows the MOFormer to intrinsically learn 3D structural information though it is not included in the input. Experiments show that pretraining improved the prediction accuracy of both models on various downstream prediction tasks. Furthermore, we revealed that MOFormer can be more data-efficient on quantum-chemical property prediction than structure-based CGCNN when training data is limited. Overall, MOFormer provides a novel perspective on efficient MOF design using deep learning.

==> MOF Transformer/zsuppinfo.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% This is a (brief) model paper using the achemso class
% %% The document class accepts keyval options, which should include
% %% the target journal and optionally the manuscript type. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \documentclass[journal=jacsat,manuscript=article]{achemso}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Place any additional packages needed here.  Only include packages
% %% which are essential, to avoid problems later. Do NOT use any
% %% packages which require e-TeX (for example etoolbox): the e-TeX
% %% extensions are not currently available on the ACS conversion
% %% servers.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage[version=3]{mhchem} % Formula subscripts using \ce{}
% \usepackage{siunitx}
% \usepackage{xspace}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage{amsfonts}
% \usepackage[utf8]{inputenc}
% \SectionNumbersOn
% \DeclareSIUnit\angstrom{\text {Å}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% If issues arise when submitting your manuscript, you may want to
% %% un-comment the next line.  This provides information on the
% %% version of every file you have used.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%\listfiles

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% Place any additional macros here.  Please use \newcommand* where
% %% possible, and avoid layout-changing macros (which are not used
% %% when typesetting).
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand*\mycommand[1]{\texttt{\emph{#1}}}
% \newcommand{\R}{\mathbb{R}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Meta-data block
%% ---------------
%% Each author should be given as a separate \author command.
%%
%% Corresponding authors should have an e-mail given after the author
%% name as an \email command. Phone and fax numbers can be given
%% using \phone and \fax, respectively; this information is optional.
%%
%% The affiliation of authors is given after the authors; each
%% \affiliation command applies to all preceding authors not already
%% assigned an affiliation.
%%
%% The affiliation takes an option argument for the short name.  This
%% will typically be something like "University of Somewhere".
%%
%% The \altaffiliation macro should be used for new address, etc.
%% On the other hand, \alsoaffiliation is used on a per author basis
%% when authors are associated with multiple institutions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\setcounter{table}{0}
\renewcommand{\tablename}{Table}
\setcounter{figure}{0}
\renewcommand{\figurename}{Figure}
% \author{Zhonglin Cao}
% \affiliation[meche]
% {Department of Mechanical Engineering, Carnegie Mellon University, Pittsburgh PA, USA 15213}
% \altaffiliation{Joint First Authorship}
% \author{Rishikesh Magar}
% \affiliation[meche]
% {Department of Mechanical Engineering, Carnegie Mellon University, Pittsburgh PA, USA 15213}
% \altaffiliation{Joint First Authorship}
% \author{Yuyang Wang}
% \affiliation[meche]
% {Department of Mechanical Engineering, Carnegie Mellon University, Pittsburgh PA, USA 15213}
% \author{Amir Barati Farimani}
% \email{barati@cmu.edu}
% \affiliation[meche]
% {Department of Mechanical Engineering, Carnegie Mellon University, Pittsburgh PA, USA 15213}
% \alsoaffiliation[biomed]
% {Department of Biomedical Engineering, Carnegie Mellon University, Pittsburgh PA, USA 15213}
% \alsoaffiliation[mld]
% {Machine Learning Department, Carnegie Mellon University, Pittsburgh PA, USA 15213}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The document title should be given as usual. Some journals require
%% a running title from the author: this should be supplied as an
%% optional argument to \title.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \title{MOFormer: Self-Supervised Transformer model for Metal-Organic Framework Property Prediction\\
% Supporting Information}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Some journals require a list of abbreviations or keywords to be
%% supplied. These should be set up here, and will be printed after
%% the title and author information, if needed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \abbreviations{IR,NMR,UV}
% \keywords{American Chemical Society, \LaTeX}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The manuscript does not need to include \maketitle, which is
%% executed automatically.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{document}
\pagenumbering{arabic}% resets `page` counter to 1
\renewcommand*{\thepage}{S\arabic{page}}
\maketitle
% \tableofcontents
\newpage
\section{Supporting Information}
\section{Self-attention and the Transformer model}
In this work, we use the encoder part of the Transformer model as the base for the MOFormer framework. Transformer\cite{vaswani2017attention} model was proposed as a language model for sequence-to-sequence language translation. The encoder part of it learns a latent representation of the input sequence using the self-attention mechanism. Self-attention mechanism is previous used along with sequential models (such as recurrent neural network\cite{bahdanau2014neural} and LSTM\cite{hochreiter1997long}) to combat the drop in model performance with long sequence. Transformer model drop the recurrent architecture in previous sequential models, and rely solely on the self-attention mechanism to learn the representation of the input sequence. The advantage of such model architecture is threefold. First, self-attention has lower per-layer computational complexity than recurrent architectures. Second, models can be highly parallelizable with only self-attention (as self-attention can be calculated using matrix multiplication) thus can be trained much faster. Third, long-range dependencies in the input sequence can be easily learned using self-attention mechanism. 

In the self-attention mechanism, each token in the sequence is linearly projected into its corresponding query, key, and value vector ($Q$, $K$, and $V$ matrix for the entire sequence, respectively). The weights that linearly project the entire input sequence are denoted as the $W_q$, $W_k$, and $W_v$ matrices. In this work, followed by Vaswani et al.\cite{vaswani2017attention}, the scaled dot-product attention:
\begin{equation}
    Attention(Q, K, V) = \text{softmax}(\frac{QK^\top}{\sqrt{d_{emb}}})V
\end{equation}
is adopted, where $d_{emb} = 512$. Multihead attention is to have multiple linear projection matrices in parallel for the calculation of attention. The $W_q$, $W_k$, and $W_v$ in each attention head is initialized differently, thus multihead attention enables the model to learn representation of the input sequence from different subspaces. Assuming we have $h$ attention heads, the multihead attention is calculated as:
\begin{equation}
\begin{split}
    Multihead Attn(Q, K, V) &= \text{Concat}(head_1 \dots head_h)W_o\\
    \text{where}\; head_i &= Attention(Q_i, K_i, V_i)
\end{split}
\end{equation}
$W_o$ is a matrix to linearly project the concatenated attention from each head; $Q_i$, $K_i$, and $V_i$ is the query, key, and value matrix of the $i$-th head, respectively. In this work, the number of head  $h=8$. The dimension of the $W_q^i$, $W_k^i$, and $W_v^i$ (linear projection matrices in the $i$-th head) is $W_q^i \in \R ^{d_{emb}\times d_k}$, $W_k^i \in \R ^{d_{emb}\times d_k}$, $W_v^i \in \R ^{d_{emb}\times d_v}$, where $d_{emb}=512$ and $d_v=d_k=d_{emb}/h=64$. Moreover, $W_o\in \R ^{d_{emb}\times d_{emb}}$.
The Transformer encoder in this work contains 6 self-attention layers (Figure 1b in the manuscript), in which the MLP has a dimension of 512.
\newpage

\section{Training Details}
In this section, we describe in details the hyperparameters that we used for training the models. Our framework consists of MOFormer (transformer), CGGNN and the SSL pretraining done to improve the performance of both the GNN and the transformer model. During the finetuning stage, a MLP regression head is attached to the encoder part (MOFormer or CGCNN) to make prediction. The regression head has 4 layers, with 512, 256, 128 and 64 neurons in each layer, respectively.

\subsection{MOFormer}
The MOFormer\textsubscript{Finetuning} hyperparameters are shown in Table~\ref{tb:PreHyperparam}. Different learning rate (LR) are used for the encoder part (Transformer encoder) and the MLP regression head. We also train the MOFormer\textsubscript{Scratch} to evaluate the improvement in performance after SSL pre-training. 

\begin{table}[htb!]
\renewcommand{\thetable}{S\arabic{table}}
  \centering
%   \small
  \resizebox{\textwidth}{!}{\begin{tabular}{l|llllllll}
    \toprule
    Hyperparameters & Batch Size & LR$_{Encoder}$ & LR$_{MLP}$ & Optimizer & Epochs & Embed. Size & Train/Val & Weight Decay \\
    \midrule
    %MOFormer\textsubscript{Pretrain}& 64 & 8 & 0.00001 & Adam & 15 & 128 &  0.95/0.05   \\
    MOFormer\textsubscript{Scratch} & 64 &  0.00005 &  0.01& Adam & 200 & 512 &  0.7/0.15/0.15  & $10^{-6}$\\
    MOFormer\textsubscript{Finetuning} & 64 &  0.00005& 0.01 & Adam & 200 & 512 &  0.7/0.15/0.15 & $10^{-6}$ \\
    \bottomrule
  \end{tabular}}
  \caption{Finetuning hyperparameters for the MOFormer model. LR indicate the learing rate}
  \label{tb:PreHyperparam}
\end{table}

\subsection{CGCNN}
The CGCNN model is structure based model that takes the ``.cif" file as input. The MOFormer is a structure agnostic method, however, information like neighbourhood of atoms and geometry of the crystal are often lost in the text representation. To ensure we also have a structure based benchmark to predict MOF properties we also evaluate the performance of the CGCNN model\cite{xie2018crystal}. The CGCNN model with its information rich features often outperforms the structure agnostic MOFormer. We also pretrain the MOFormer and the CGCNN together using the self-supervised learning. The performance of pretrained CGCNN\textsubscript{Pretrain} model is found to be higher than CGCNN\textsubscript{Scratch} model trained from Scratch without pretraining. The hyperparamters we used for the model are shown in Table~\ref{tb:PreHyperparamCG}.

\begin{table}[htb!]
\renewcommand{\thetable}{S\arabic{table}}
  \centering
%   \small
  \resizebox{\textwidth}{!}{\begin{tabular}{l|llllllll}
    \toprule
    Hyperparameters & Batch Size &Number of layers & LR & Optimizer & Epochs & Embed. Size & Train/Val/Test & Weight Decay \\
    \midrule
    %MOFormer\textsubscript{Pretrain}& 64 & 8 & 0.00001 & Adam & 15 & 128 &  0.95/0.05   \\
    CGCNN\textsubscript{Scratch} & 128 & 3 &  0.01 & Adam & 200 & 512 &  0.7/0.15/0.15  & $10^{-6}$ \\
    CGCNN\textsubscript{Finetuning}& 128 & 3 &  0.002 & Adam & 200 & 512 &  0.7/0.15/0.15  &  $10^{-6}$\\
    \bottomrule
  \end{tabular}}
  \caption{Finetuning hyperparameters for the CGCNN model. LR denotes the learning rate for the models.}
  \label{tb:PreHyperparamCG}
\end{table}

\subsection{SSL - Pretraining}
Structure agnostic models often lack the geometry and atom neighborhood information leading to an information bottleneck for these models. To mitigate this issue, we develop the SSL pre-training framework. In the SSL pre-training framework we have the MOFormer branch and the CGCNN branch, the goal of the SSL pre-training is to ensure that the representations from both the MOFormer and the CGCNN are similar. The pre-training helps both the MOFormer model and CGCNN in a way that it tries to leverage the embeddings learnt by the other model. The model benefit mutually from each other and the performance enhancements can be seen for both models during the finetuning stage (Figure ~\ref{fig:ssl_mof}). The hyperparamters we used during pretraining the model are shown in  Table ~\ref{tb:PreHyperparamPre}
\begin{table}[htb!]
\renewcommand{\thetable}{S\arabic{table}}
  \centering
%   \small
  \resizebox{\textwidth}{!}{\begin{tabular}{l|llllllll}
    \toprule
    Hyperparameters & Batch Size & Learning Rate & Optimizer & Epochs & Embed. Size & Train/Val \\
    \midrule
    %MOFormer\textsubscript{Pretrain}& 64 & 8 & 0.00001 & Adam & 15 & 128 &  0.95/0.05   \\
    CGCNN\textsubscript{Pretrain} & 32 &  0.00001 & Adam & 15 & 512 &  0.95/0.05   \\
    MOFormer\textsubscript{Pretrain}& 32 &  0.00001 & Adam & 15 & 512 &  0.95/0.05   \\
    \bottomrule
  \end{tabular}}
  \caption{Hyperparameters for Pretraining the model.}
  \label{tb:PreHyperparamPre}
\end{table}

\begin{figure}[htb!]
\renewcommand{\thefigure}{S\arabic{figure}}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/SSL_MOF.pdf}
    \caption{The SSL pretraining and finetuning framework. In this work, we use self supervised learning to pre-train both the CGCNN model and the MOFormer using self-supervised learning. The pre-trained weights are then shared during finetuning for down stream tasks. Using such a technique help us improve the perfromance of both the CGCNN and MOFormer. }
    \label{fig:ssl_mof}
\end{figure}

\newpage

\section{Distribution of the benchmark datasets}
Since only part of MOF in each QMOF\cite{rosen2021machine} and hMOF\cite{wilmer2012large} dataset have available MOFid, we plot the distribution of the whole datasets and the subsets with MOFid. Figure~\ref{fig:qmof_dist} shows that the difference between the average band gap value between the whole dataset and the subset is as small as 0.135. The distribution between the data are also similar.

Figure~\ref{fig:hmof_dist} shows that the difference between the average \ce{CO_2}/\ce{CH_4} adsorption value between the whole dataset and the subset is very small. The distribution between the data are also similar. Therefore the benchmark results comparisons between MOFormer and other models on both datasets are fair.
\begin{figure}[htb!]
\renewcommand{\thefigure}{S\arabic{figure}}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/qmof_dist.png}
    \caption{Histogram showing the distribution of QMOF dataset. Blue bars are all MOFs in the QMOF dataset. Orange bars are MOFs with MOFid available. Mean $\mu$ and standard deviation $\sigma$ are reported.}
    \label{fig:qmof_dist}
\end{figure}

\begin{figure}[htb!]
\renewcommand{\thefigure}{S\arabic{figure}}
    \centering
    \includegraphics[width=\linewidth]{figs/hmof_dist.pdf}
    \caption{Histogram showing the distribution of hMOF dataset with the label of \textbf{(a)} \ce{CO_2} adsoprtion and \textbf{(b)} \ce{CH_4} adsorption at 0.05, 0.5, and 2.5 bar of pressure. Blue bars are all MOFs in the hMOF dataset. Orange bars are MOFs with MOFid available. Mean $\mu$ and standard deviation $\sigma$ are reported.}
    \label{fig:hmof_dist}
\end{figure}

\newpage

\section{Parameters to create SOAP feature vector}
The SOAP\cite{bartok2013representing} feature vector is created using the DScribe package\cite{dscribe}. Table~\ref{tb:soap} records the parameters for creating SOAP feature vector, which are chosen arbitrarily based on previous works\cite{fung2021benchmarking, rosen2021machine}.

\begin{table}[htb!]
\renewcommand{\thetable}{S\arabic{table}}
  \centering
  \small
  \begin{tabular}{llllll}
    \toprule
    rcut & $\sigma$ & nmax & lmax & average method & crossover\\
    \midrule
    8& 0.2 & 8 & 6 & Inner average & False   \\
    \bottomrule
  \end{tabular}
  \caption{Parameters used for creating SOAP feature vector}
  \label{tb:soap}
\end{table}

The length of the SOAP feature vector varies greatly based on the number of different atom elements in the dataset. When the MOFs in a dataset includes a large variation of elements (such as QMOF, 79 elements), the SOAP feature vector will be very long and sparse. However, when the MOFs in the dataset consist of only a few different elements (such as hMOF, 11 elements), the SOAP feature vector will be relatively short and less sparse. For example, SOAP feature vector created using the 11 elements in hMOF has a length of 2772. The SOAP feature vector created using the 79 elements in QMOF has a length of 19908, given that nmax and lmax parameters are kept the same. The high accuracy of SOAP feature vector on hMOF is a direct result of the small variation of element type in the dataset. Assuming that we create the SOAP feature vectors for hMOFs using double the original number of elements (22 instead of the original 11), the length of SOAP feature vector will be doubled to 5544. The performance of XGBoost using the new SOAP feature is significantly reduced (Table~\ref{tb:soap2}). Therefore, we can conclude that SOAP feature is not a suitable choice when exploring the chemical space for MOFs where elements are diverse.

\begin{table}[htb!]
\renewcommand{\thetable}{S\arabic{table}}
  \centering
  \small
  \begin{tabular}{llll}
    \toprule
    Model & $\#$ elements & SOAP vector length & hMOF 2.5 bar \ce{CH_4} adsorption \\
    \midrule
    SOAP& 11 & 2772 & 0.239$\pm$0.002  \\
    SOAP& 22 & 5544& 0.288$\pm$0.002   \\
    CGCNN\textsubscript{pretrain}& - & - & 0.258$\pm$0.008   \\
    \bottomrule
  \end{tabular}
  \caption{Parameters used for creating SOAP feature vector}
  \label{tb:soap2}
\end{table}
\newpage
\section{Comparison between models' performance in QMOF dataset}
Figure~\ref{fig:qmof_kde} shows the kernel density estimation (KDE) plot of the predicted band gap values of MOFs from different models. The MOFs are in a randomly selected test set from the QMOF dataset. The ground truth is the DFT calculated band gap, which is shown by the blue curve. SOAP and Stoichiometric-120 features with XGBoost model underpredict low bandgap values more frequently than CGCNN and MOFormer.
\begin{figure}[htb!]
\renewcommand{\thefigure}{S\arabic{figure}}
    \centering
    \includegraphics[width=\linewidth]{figs/qmof_kde.pdf}
    \caption{\textbf{(a)} The kernel density estimation (KDE) plot of the predicted band gap values of MOFs from different models. \textbf{(b)} Zoom-in view of the distribution of MOFs with band gap $\leq$ 1eV}
    \label{fig:qmof_kde}
\end{figure}
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The appropriate \bibliography command should be placed here.
%% Notice that the class file automatically sets \bibliographystyle
%% and also names the section correctly.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
% \bibliography{ref}

% \end{document}
